HalOmi: A Manually Annotated Benchmark for Multilingual Hallucination and Omission Detection in Machine Translation

Hallucinations in machine translation are translations that contain information completely unrelated to the input. Omissions are translations that do not include some of the input information. While both cases tend to be catastrophic errors undermining user trust, annotated data with these types of pathologies is extremely scarce and is limited to a few high-resource languages. In this work, we release an annotated dataset for the hallucination and omission phenomena covering 18 translation directions with varying resource levels and scripts. Our annotation covers different levels of partial and full hallucinations as well as omissions both at the sentence and at the word level. Additionally, we revisit previous methods for hallucination and omission detection, show that conclusions made based on a single language pair largely do not hold for a large-scale evaluation, and establish new solid baselines.

==> old_neurips_files/perturbed_backup.tex <==
\section{Artificially induced pathologies}
\label{sect:natural_vs_perturbed}

\paragraph{Motivation.} Even after pre-selecting translations with detection methods, the proportion of hallucinations for high-resource languages is low. To increase their number, we tried different methods of perturbing the translations. A good perturbation method would produce a lot of pathologies, which are not too unlikely from the point of view of an unperturbed model. 
\david{TODO: say more diplomatically that the best perturbation method that we tried still turned out to be inadequate.} We tried to come up with such a method, but in the end it turned out to be inadequate for evaluating detection methods.

\paragraph{Methods of perturbation.} 
We compared regular translations (\texttt{base}) with multiple perturbations: replacing the whole translation with a randomly chosen sentence (\texttt{permuting}), leaving dropout on during inference (\texttt{dropout}), sampling the next tokens from the predicted distribution with different temperatures instead of beam search (\texttt{sample}), inserting the ``unknown'' token into the source sentence (\texttt{unk}), and our novel method, \texttt{detaching}. This last method decreases the output activations of all the encoder-decoder attention layers by a constant multiplier $\alpha$, imitating natural detaching hallucinations. For \texttt{dropout}, \texttt{sample} and \texttt{detaching}, we tried several values of the parameters controlling the perturbation strength.

\begin{figure}[h!]
  \centering
   \includegraphics[width=12cm]{figures/comparing_perturbations}
  \caption{Comparing the methods of perturbing translation \david{re-generate the image with new labels}}
  \label{fig:perturb_tradeoff}
\end{figure}


\paragraph{Evaluating perturbation methods.} We translate the FLORES dev subset between English and 5 other high-resource languages using all perturbation methods. We approximate the proportion of pathologies with a portion of translation with LaBSE cosine similarity to the source below 0.75, and their unnaturalness with the Seq-Logprob of the unperturbed model. Figure \ref{fig:perturb_tradeoff} shows these qualities, averaged over translation directions, for each perturbation method. The \texttt{detaching} methods seems to reach the best tradeoff of pathology frequency and naturalness. Therefore, for the following experiments, we use only this perturbation method, with the $\alpha=0.3$ value that results in the average Seq-logprob similar to that of reference translations.

\paragraph{Applicability of perturbed translations.}

We applied exactly the same filtering, annotation and post-processing to the detached translations as to the natural ones (Section \ref{sec:creation}). The manual annotation of these translations demonstrated very high hallucination rates for all directions, so we initially intended to include them in the final dataset. However, after collecting all the annotations, we discovered that the perturbed translations are unsuitable for benchmarking detection methods, because they produce a different ranking of methods than the natural translations. 

Table \ref{tab:perturbed} shows the evaluation scores for different methods of hallucination and omission detection on all translation directions.\footnote{For comparability, we downsampled the data so that on the natural and perturbed subsets have equal number of observations for each combination of pathology type, source dataset and translation direction.} We can see that perturbing the translation model introduces biases into the evaluation of detection methods. For example, on the natural translations, SeqLogprob outperforms ALTI as a hallucination detector, while on the perturbed translations, the opposite is true. 



\begin{table}[h!]
  \caption{\% of correctly ranked pairs for detection on natural and perturbed translations, averaged over translation directions. H: hallucinations, O: omissions (on the data without hallucinations), nat: natural subset, per: perturbed subset.}
  \label{tab:perturbed}
  \centering

\begin{tabular}{lrrrr}
 & H, nat & H, per & O, nat & O, per \\
 \hline
Seq-Logprob & {\cellcolor[HTML]{3B92C1}} \color[HTML]{F1F1F1} 0.81 & {\cellcolor[HTML]{6DA6CD}} \color[HTML]{F1F1F1} 0.76 & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} 0.58 \\
ALTI & {\cellcolor[HTML]{5C9FC9}} \color[HTML]{F1F1F1} 0.77 & {\cellcolor[HTML]{2685BB}} \color[HTML]{F1F1F1} 0.83 & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} 0.47 & {\cellcolor[HTML]{FEF6FA}} \color[HTML]{000000} 0.51 \\
ALTI-T & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} 0.58 & {\cellcolor[HTML]{BCC7E1}} \color[HTML]{000000} 0.65 & {\cellcolor[HTML]{65A3CB}} \color[HTML]{F1F1F1} 0.76 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 0.61 \\
Attn-OT & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} 0.50 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} 0.65 & {\cellcolor[HTML]{C8CDE4}} \color[HTML]{000000} 0.64 \\
COMET-QE & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{8BB2D4}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} 0.50 & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} 0.58 \\
LaBSE & {\cellcolor[HTML]{3991C1}} \color[HTML]{F1F1F1} 0.81 & {\cellcolor[HTML]{2786BB}} \color[HTML]{F1F1F1} 0.83 & {\cellcolor[HTML]{A9BFDC}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{D9D8EA}} \color[HTML]{000000} 0.60 \\
LASER & {\cellcolor[HTML]{7EADD1}} \color[HTML]{F1F1F1} 0.74 & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} 0.73 & {\cellcolor[HTML]{D5D5E8}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{E0DDED}} \color[HTML]{000000} 0.59 \\
XNLI & {\cellcolor[HTML]{BBC7E0}} \color[HTML]{000000} 0.66 & {\cellcolor[HTML]{ABBFDC}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} 0.59 & {\cellcolor[HTML]{B0C2DE}}  0.67 \\
\hline
\end{tabular}


\end{table}


Therefore, we do not recommend using perturbed translations for comparing the methods of hallucination or omission detection. Nevertheless, the techniques of generating untrustworthy translations may be applied, for example, to generate synthetic data for pretraining supervised hallucination detection models (that still should be evaluated later with natural translations).

